Diffscaler: Enhancing the Generative Prowess of Diffusion Transformers

Recently, diffusion transformers have gained wide attention with its excellent performance in text-to-image and text-to-vidoe models, emphasizing the need for transformers as backbone for diffusion models. Transformer-based models have shown better generalization capability compared to CNN-based models for general vision tasks. However, much less has been explored in the existing literature regarding the capabilities of transformer-based diffusion backbones and expanding their generative prowess to other datasets. This paper focuses on enabling a single pre-trained diffusion transformer model to scale across multiple datasets swiftly, allowing for the completion of diverse generative tasks using just one model. To this end, we propose DiffScaler, an efficient scaling strategy for diffusion models where we train a minimal amount of parameters to adapt to different tasks. In particular, we learn task-specific transformations at each layer by incorporating the ability to utilize the learned subspaces of the pre-trained model, as well as the ability to learn additional task-specific subspaces, which may be absent in the pre-training dataset. As these parameters are independent, a single diffusion model with these task-specific parameters can be used to perform multiple tasks simultaneously. Moreover, we find that transformer-based diffusion models significantly outperform CNN-based diffusion models methods while performing fine-tuning over smaller datasets. We perform experiments on four unconditional image generation datasets. We show that using our proposed method, a single pre-trained model can scale up to perform these conditional and unconditional tasks, respectively, with minimal parameter tuning while performing as close as fine-tuning an entire diffusion model for that particular task.

==> ablation_expts/adaptor_dim.tex <==
\begin{table}[t]
\centering

\scalebox{0.8}{
\begin{tabular}{c| c}
\toprule
dim&FID&IS\\
\midrule
1 && \\
4&&\\
8&&\\
16 &&\\
32 &&\\
64&&\\
256&&
\bottomrule
\end{tabular}
}
\caption{}
\label{tab:adadim}
\vspace{-3mm}
\end{table}


==> ablation_expts/adaptor_layers_down_up.tex <==
\begin{table}[t]
\centering

\scalebox{0.8}{
\begin{tabular}{c| c}
\toprule
dim&FID&IS\\
\midrule
28-24 && \\
28-20&&\\
28-16&&\\
28-12 &&\\
28-8 &&\\
28-4&&\\
28-1&&
\bottomrule
\end{tabular}
}
\caption{}
\label{tab:adadim}
\vspace{-3mm}
\end{table}


==> ablation_expts/adaptor_layers_up_down.tex <==
\begin{table}[t]
\centering

\scalebox{0.8}{
\begin{tabular}{c| c}
\toprule
dim&FID&IS\\
\midrule
1-4 && \\
1-8&&\\
1-12&&\\
1-16 &&\\
1-20 &&\\
1-24&&\\
1-28&&
\bottomrule
\end{tabular}
}
\caption{}
\label{tab:adadim}
\vspace{-3mm}
\end{table}


==> ablation_expts/batch_size.tex <==
\begin{table}[t]
\centering

\scalebox{0.8}{
\begin{tabular}{c| c}
\toprule
dim&FID&IS\\
\midrule
16 && \\
32&&\\
64&&\\
128&&\\
256&&\\
512&&\\
\bottomrule
\end{tabular}
}
\caption{}
\label{tab:adadim}
\vspace{-3mm}
\end{table}


==> ablation_expts/bias_norm_layers_down_up.tex <==
\begin{table}[t]
\centering

\scalebox{0.8}{
\begin{tabular}{c| c}
\toprule
dim&FID&IS\\
\midrule
28-24 && \\
28-20&&\\
28-16&&\\
28-12 &&\\
28-8 &&\\
28-4&&\\
28-1&&
\bottomrule
\end{tabular}
}
\caption{}
\label{tab:adadim}
\vspace{-3mm}
\end{table}


==> ablation_expts/bias_norm_up_down.tex <==
\begin{table}[t]
\centering

\scalebox{0.8}{
\begin{tabular}{c| c}
\toprule
dim&FID&IS\\
\midrule
1-4 && \\
1-8&&\\
1-12&&\\
1-16 &&\\
1-20 &&\\
1-24&&\\
1-28&&
\bottomrule
\end{tabular}
}
\caption{}
\label{tab:adadim}
\vspace{-3mm}
\end{table}


==> ablation_expts/decoder_num.tex <==
\begin{table}[t]
\centering

\scalebox{0.8}{
\begin{tabular}{c| c}
\toprule
dim&FID&IS\\
\midrule
1 && \\
2&&\\
3&&\\
4 &&\\
8&&\\
14&&


\bottomrule
\end{tabular}
}
\caption{}
\label{tab:adadim}
\vspace{-3mm}
\end{table}


==> ablation_expts/mask_ratio.tex <==
\begin{table}[t]
\centering

\scalebox{0.8}{
\begin{tabular}{c| c}
\toprule
dim&FID&IS\\
\midrule
0.1 && \\
0.2&&\\
0.3&&\\
0.4 &&\\
0.5 &&\\
0.6&&\\
0.7 && \\
0.8&&\\
0.9&&\\
1.0 &&\\

\bottomrule
\end{tabular}
}
\caption{}
\label{tab:adadim}
\vspace{-3mm}
\end{table}


==> ablation_expts/weight_layers_down_up.tex <==
\begin{table}[t]
\centering

\scalebox{0.8}{
\begin{tabular}{c| c}
\toprule
dim&FID&IS\\
\midrule
28-24 && \\
28-20&&\\
28-16&&\\
28-12 &&\\
28-8 &&\\
28-4&&\\
28-1&&
\bottomrule
\end{tabular}
}
\caption{}
\label{tab:adadim}
\vspace{-3mm}
\end{table}


==> ablation_expts/weight_layers_up_down.tex <==
\begin{table}[t]
\centering

\scalebox{0.8}{
\begin{tabular}{c| c}
\toprule
dim&FID&IS\\
\midrule
1-4 && \\
1-8&&\\
1-12&&\\
1-16 &&\\
1-20 &&\\
1-24&&\\
1-28&&
\bottomrule
\end{tabular}
}
\caption{}
\label{tab:adadim}
\vspace{-3mm}
\end{table}


==> metrics/ablation.tex <==

\begin{table}[t]
\vspace{-.2em}
\centering
%#################################################
% VideoMAE decoder depth
%#################################################
\subfloat[
\textbf{Role of a,b,s}.
\label{tab:decoder_depth}
]{
\centering
\begin{minipage}{0.28\linewidth}{\begin{center}
\tablestyle{2pt}{1.05}
\begin{tabular}{x{20}x{23}x{20}x{40}}
blocks & SSV2 & CNN & DiT.  \\
\shline
a &  68.5 & 79.0 & 7.9G \\ 
b &  69.2 & 79.2 & 10.2G \\
w & \baseline{\textbf{69.6}} & \baseline{\textbf{80.0}} & 14.7G \\
% 8 & 69.3 & 79.7 & 23.7G \\
\end{tabular}
\end{center}}\end{minipage}
}
\hspace{2em}
\subfloat[
\textbf{Role pf d}. Role of masking ratio
\label{tab:mask_types}
]{
\begin{minipage}{0.27\linewidth}{\begin{center}
\tablestyle{2pt}{1.05}
\begin{tabular}{y{26}x{24}x{22}x{22}}
case & ratio & SSV2 & K400 \\
\shline
tube & 75 & 68.0 & 79.8 \\
tube & 90 & \baseline{\textbf{69.6}} &  \baseline{\textbf{80.0}} \\
random & 90 & 68.3 & 79.5 \\
frame & 87.5$^*$ &  61.5 & 76.5 \\
\end{tabular}
\end{center}}\end{minipage}
}
\hspace{1.5em}
%#################################################
% VideoMAE targets
%#################################################
\subfloat[
\textbf{Role of s}. Role of weight basis.
\label{tab:abl_target}
]{
\begin{minipage}{0.28\linewidth}{\begin{center}
\tablestyle{4pt}{1.05}
\begin{tabular}{x{20}x{26}x{20}x{20}}
input & target & SSV2 & K400 \\
\shline
$T$\x$\tau$ & $\emph{center}$ & 63.0 &  79.3 \\
$T$\x$\frac{\tau}{2}$ & $T$\x$\frac{\tau}{2}$ & 68.9 &  79.8  \\
$T$\x$\tau$ & $T$\x$\tau$ &  \baseline{\textbf{69.6}} & \baseline{80.0} \\
$T$\x$\tau$ & $2T$\x$\frac{\tau}{2}$ &  69.2 &  \textbf{80.1} \\
\end{tabular}
\end{center}}
\end{minipage}
}
\\
\centering
% \vspace{-0.6em}

%#################################################
% VideoMAE pre-training strategy
%#################################################
\hspace{-1.5em}
\subfloat[
\textbf{Pre-training strategy}. Our VideoMAE works the best without using any extra data. ``sup.'' is supervised training.
\label{tab:abl_pretrain}
]{
\centering
\begin{minipage}{0.29\linewidth}{\begin{center}
\tablestyle{2pt}{1.05}
\begin{tabular}{y{68}x{20}x{20}}
case & SSV2 & K400 \\
\shline
\emph{from scratch}  & 32.6 & 68.8 \\
ImageNet-21k sup.  & 61.8 & 78.9 \\
IN-21k+K400 sup. & 65.2 & - \\
VideoMAE  & \baseline{\textbf{69.6}} & \baseline{\textbf{80.0}} \\
\end{tabular}
\end{center}}\end{minipage}
}
\hspace{1em}
%#################################################
% VideoMAE pre-training dataset
%#################################################
\subfloat[
\textbf{Pre-training dataset}. Our VideoMAE works the best when directly pre-training the models on the source datasets.
\label{tab:abl_dataset}
]{
\centering
\begin{minipage}{0.29\linewidth}{\begin{center}
\tablestyle{2pt}{1.05}
\begin{tabular}{x{24}x{39}x{21}x{19}}
dataset & method & SSV2 & K400 \\
\shline
IN-1K &  ImageMAE & 64.8 & 78.7 \\
K400 &  VideoMAE & 68.5 & \baseline{\textbf{80.0}} \\
SSV2 &  VideoMAE  & \baseline{\textbf{69.6}} & 79.6 \\
\multicolumn{4}{c}{~} \\
\end{tabular}
\end{center}}\end{minipage}
}
\hspace{1.5em}
%#################################################
% VideoMAE loss function
%#################################################
\subfloat[
\textbf{Loss function}. MSE loss works the best for the masking and reconstruction task in VideoMAE.
\label{tab:abl_loss}
]{
\begin{minipage}{0.26\linewidth}{\begin{center}
\tablestyle{2pt}{1.05}
\begin{tabular}{y{58}x{22}x{22}}
case & SSV2 & K400 \\
\shline
L1 loss  & 69.1 & 79.7 \\
MSE loss & \baseline{\textbf{69.6}} & \baseline{\textbf{80.0}} \\
Smooth L1 loss  & 68.9 & 79.6 \\
\multicolumn{3}{c}{~}\\
\end{tabular}
\end{center}}\end{minipage}
}
% \vspace{-.5em}
\caption{Ablation experiments. 
}
\label{tab:ablations} 
\vspace{-2.5em}
\end{table}

==> metrics/ablation_table_CNN.tex <==

\begin{table}[ht]
\vspace{-1.0em}
% \begin{center}
\centering
\caption{Ablation Experiments}\label{tab:ablations}
\subfloat[
Individual components\label{tab:insert_form}
]{
\begin{minipage}{0.3\textwidth}{\begin{center}
\tablestyle{0.1pt}{1.33}
\begin{tabular}{y{35}x{35}x{35}x{20}}
\Xhline{1.0pt}
layers & \#params & FID &IS \\
\hline
b  &0.48M& 105.04&5.88 \\
a&0.48M&349.19& 2.22\\
 % &&18.25& 4.35 \\
$W_{up}$ &47.7 M&36.48& 4.82\\
$W_{up}$ \& s&47.7M&71.81&5.81 \\ 
\Xhline{1.0pt}
\end{tabular}
\end{center}}

\end{minipage}
}
\subfloat[
Latent dimension $d$\label{tab:s_factor}
]{
\begin{minipage}{0.3\textwidth}{\begin{center}
\tablestyle{3pt}{1.33}
\begin{tabular}{x{20}x{30}x{20}x{20}}
\Xhline{1.0pt}
dim  & \#params &FID&IS \\
\hline
1 &0.77M &99.24&14.79  \\
4 & 3.01M&78.55&6.62 \\
16&11.9M &89.51 &7.75 \\
32&48.7M&71.81&5.81  \\
\Xhline{1.0pt}
\end{tabular}
\end{center}}\end{minipage}
}
% \subfloat[
% Mask ratio $M$\label{tab:s_factor}
% ]{
% \begin{minipage}{0.3\textwidth}{\begin{center}
% \tablestyle{3pt}{1.33}
% \begin{tabular}{x{20}x{20}x{20}x{40}}
% \Xhline{1.0pt}
% ratio &FID & IS& GFLOPS \\
% \hline
% 0.75 & 98.88&2.85& 34.4 \\
% 0.50 & 37.31 &3.46& 68.8 \\
% 0.25 & 17.28 & 3.97&103.2 \\
% 0.00&19.13&4.72 &137.6 \\
% \Xhline{1.0pt}
% \end{tabular}
% \end{center}}\end{minipage}
% }
\newline
\label{abl}
\end{table}



% %##################################################################################################
% % overall table of all ablations
% \begin{table}[ht]
% \vspace{-1.0em}
% % \begin{center}
% \centering
% \caption{\textbf{\ourabbr ablation experiments} with ViT-B/1}\label{tab:ablations}
% %#################################################
% % Hidden Dimension
% %#################################################
% \subfloat[
% \textbf{Middle dimension $\hat{d}$.}\label{tab:hidden_dim}
% ]{
% \begin{minipage}{0.3\textwidth}
% {\begin{center}
% \tablestyle{2pt}{1.13}
% \begin{tabular}{x{40}x{30}x{30}}
% \Xhline{1.0pt}
% mid dim &  \#params& top-1 \\
% \hline
% 1   & 0.16M & 50.03 \\
% 16  & 0.44M & 57.62 \\
% 32  & 0.73M & 58.27 \\
% \bestcell{64}  & \bestcell{1.32M} & \bestcell{\textbf{59.02}} \\
% 256 & 4.87M & 58.87 \\
% \Xhline{1.0pt}
% \end{tabular}
% \end{center}}\end{minipage}
% }
% \subfloat[
% \textbf{AdaptMLP inserted layers and form.}\label{tab:insert_form}
% ]{
% \begin{minipage}{0.4\textwidth}{\begin{center}
% \tablestyle{0.1pt}{1.33}
% \begin{tabular}{y{40}x{40}x{30}x{30}}
% \Xhline{1.0pt}
% layers & form & \#params & top-1 \\
% \hline
% 1 $\rightarrow$ 6 & parallel & 0.73 & 50.48 \\
% 7 $\rightarrow$ 12 & parallel  & 0.73 & 57.99 \\
% \bestcell{1 $\rightarrow$ 12} & \bestcell{parallel} & \bestcell{1.32} & \bestcell{59.02} \\
% 1 $\rightarrow$ 12 & sequential & 1.32 & 58.17 \\
% \Xhline{1.0pt}
% \end{tabular}

% \end{center}}
% \vspace{-1.5em}
% \end{minipage}
% }
% %#################################################
% % Scaling factor s
% %#################################################
% \subfloat[
% \textbf{Scaling factor $s$.}\label{tab:s_factor}
% ]{
% \begin{minipage}{0.3\textwidth}{\begin{center}
% \tablestyle{3pt}{1.33}
% \begin{tabular}{x{20}x{30}}
% \Xhline{1.0pt}
% factor & top-1 \\
% \hline
% 0.01 & 53.44 \\
% 0.05 & 58.85 \\
% \bestcell{0.10} & \bestcell{59.02} \\
% 0.20 & 58.89 \\
% \Xhline{1.0pt}
% \end{tabular}
% \end{center}}\end{minipage}
% }
% \end{table}
% %##################################################################################################
% % overall table of all ablations

==> metrics/compariosn.tex <==


\begin{table*}[htbp]
\centering
\begin{center}
\vspace{-2mm}
% \setlength{\tabcolsep}{6pt}
\scalebox{1}{
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c| c| c c |c c |c c |c c|  }
\toprule
%\rowcolor{color3} 
%\rowcolor{color3} 
% \multirow{3}{*}{Method}&\multicolumn{7}{c}{Stable Diffusion}\\
% \cmidrule(lr){2-10} 
\multirow{2}{*}{Method}
  &\multirow{2}{*}{Parameters} & \multicolumn{2}{c}{Hed}&\multicolumn{2}{c}{Depth}  &\multicolumn{2}{c}{Segmentation Map} &\multicolumn{2}{c}{ Canny} \\
  \cmidrule(lr){3-10}
&&FID$(\downarrow)$&CLIP$(\uparrow)$ & FID$(\downarrow)$&CLIP$(\uparrow)$ &FID$(\downarrow)$&CLIP$(\uparrow)$ &FID$(\downarrow)$&CLIP$(\uparrow)$ \\
\midrule
ControlNet \cite{zhang2023adding} & 361.2 M (33\%)& 20.99 &152.03 & 22.09&151.15 &27.56 &76.18 &19.22 &\bestcell{150.59}   \\
DiffScaler & 6.85 M (0.5\%)& \bestcell{16.82}&\bestcell{155.26} &\bestcell{17.82} &\bestcell{153.34} &\bestcell{19.30}  &\bestcell{144.21}& \bestcell{15.80} &149.46   \\
\bottomrule
\end{tabular}
}
}
\end{center}
% \vspace{-1.5em}
\caption{Quantitative comparisons for conditional sampling.}
\label{table:cond}
\end{table*}



% \begin{table*}[!t]
% \begin{center}
% \label{table:inpaint}
% \vspace{-2mm}
% % \setlength{\tabcolsep}{6pt}
% \scalebox{0.9}{

% \begin{tabular}{c c c c c c c c c c c c }
% \toprule
% %\rowcolor{color3} 
% %\rowcolor{color3} 
% \multirow{2}{*}{Method}&\multicolumn{5}{c}{Guided-Diffusion}&\multicolumn{5}{c}{DiT}\\
% \cmidrule(lr){2-6} \cmidrule(lr){7-11} 
%    & CUB &  Flowers &FFHQ &Food &Caltech&   CUB &  Flowers &FFHQ&Food&Caltech \\

% \midrule
% Full-tuning & & & & & & & & & & &  \\
% Fine-Tuning & & & & & & & & & & &  \\
% LORA & & & & & & & & & & &  \\
% BitFit & & & & & & & & & & &  \\
% Ours & & & & & & & & & & &  \\
% \bottomrule
% \end{tabular}
% }
% \end{center}

% % \vspace{-1.5em}
% \caption{Quantitative Comparisons for unconditional sampling.}
% \end{table*}

==> metrics/conditonal_comparison_CNN.tex <==


\begin{table*}[htbp]
\begin{center}
\vspace{-2mm}
% \setlength{\tabcolsep}{6pt}
\scalebox{1}{
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c| c| c c |c c |c c |c c| c c| }
\toprule
%\rowcolor{color3} 
%\rowcolor{color3} 
% \multirow{3}{*}{Method}&\multicolumn{9}{c}{Diffusion Transformer}\\
% \cmidrule(lr){2-12} 
\multirow{2}{*}{Method}
  &\multirow{2}{*}{Parameters} & \multicolumn{2}{c}{CUB}&\multicolumn{2}{c}{Flowers}  &\multicolumn{2}{c}{FFHQ}  &\multicolumn{2}{c}{Food} &\multicolumn{2}{c}{ Caltech} \\
  \cmidrule(lr){3-12}
% &&CLI&IS & FID&IS &FID&IS &FID&IS &FID&IS \\
&&$FID$$(\downarrow)$&IS$(\uparrow)$& $FID(\downarrow)$&IS$(\uparrow)$ &$FID(\downarrow)$&IS$(\uparrow)$&$FID(\downarrow)$&IS$(\uparrow)$&$FID(\downarrow)$&IS$(\uparrow)$ \\
\midrule
% Fine-Tuning & 674M & 18.30&5.15 &20.07 &3.38 &15.50 &4.37 &14.46 &4.13 & 45.99&14.35    \\
% \midrule
% LORA & 47.7 M&30.97 &\bestcell{6.09} &18.75 &3.42 & 22.46 &4.50&\bestcell{19.65} &4.13 &52.42 &11.58 \\
% BitFit &0.48M&\bestcell{19.75} &4.93 & 23.94& \bestcell{3.61}&30.00 &4.70 &22.90 &4.34 & 54.93& 12.32  \\
% Adaptformer &&28.81&6.84&15.44&3,71&16.47&4.08& 20.82&4.44 &53.49 &12.97 \\
DiffScaler(Parallel)&48.7M &20.19 &5.03 &18.07 &3.50 &15.13&4.70 &31.33&4.56 &51.46 &13.76   \\
DiffScaler(Sequential)&48.7M &20.19 &5.03 &21.58 &3.73 &36.73&3.84  &39.21&5.24 &97.58 &10.33  \\
DiffScaler(CNN backbone)&48.7M &25.23 &4.81 &59.15 &4.38 &77.88&5.95  &35.23&4.81 &92.43 &9.76  \\
% Ours-Scale &&14.90 &5.20 &21.58 &3.37 &36.73 & 3.84  &39.21&5.24 &97.58 &10.33  \\
\bottomrule
\end{tabular}
}
}
\end{center}
% \vspace{-1.5em}
\caption{Quantitative comparisons for unconditional sampling. The first two rows correspond to the parallel and sequential configuration of DiT backbone while using DiffScaler. Sequential corresponds to scaling by adding new datasets one by one in the order of CUB, Flowers, FFHQ, Food, and Caltech. Parallel corresponds to training the models separately and then stacking the parameters. }
\label{table:uncond}
\end{table*}

==> tex_files/unconditional.tex <==
\begin{figure*}
    \centering
    \setlength{\tabcolsep}{0.5pt}
    {\small
    \renewcommand{\arraystretch}{0.5} 
    \begin{tabular}{c c c c c c c c c c c c}
    \captionsetup{type=figure, font=scriptsize}
    \hspace{-2mm}
    \raisebox{0.15in}{\rotatebox{90}{\scriptsize \emph{A yellow}
 }}
    \vspace{0.1cm}
            \textit{(b) Incremental Class Conditioning} \\
\raisebox{0.25in}{\rotatebox{90}{\scriptsize \textit{FFHQ}
 }}
 \includegraphics[width=0.094\linewidth]{introfig/uncond/faces/1.jpg}
 \includegraphics[width=0.094\linewidth]{introfig/uncond/faces/4.jpg}
 \includegraphics[width=0.094\linewidth]{introfig/uncond/faces/5.jpg}
 \includegraphics[width=0.094\linewidth]{introfig/uncond/faces/9.jpg}
 \includegraphics[width=0.094\linewidth]{introfig/uncond/faces/10.jpg}
 \hspace{2mm}
 \raisebox{0.15in}{\rotatebox{90}{\scriptsize \textit{CUB-200}
 }}
  \includegraphics[width=0.094\linewidth]{introfig/uncond/birds/2.jpg}
 \includegraphics[width=0.094\linewidth]{introfig/uncond/birds/3.jpg}
 \includegraphics[width=0.094\linewidth]{introfig/uncond/birds/4.jpg}
 \includegraphics[width=0.094\linewidth]{introfig/uncond/birds/8.jpg}
  \includegraphics[width=0.094\linewidth]{introfig/uncond/birds/9.jpg}
     \tabularnewline
% \hspace{-2mm}
 \raisebox{0.05in}{\rotatebox{90}{\scriptsize \textit{FLOWERS-101}
 }}
 \includegraphics[width=0.094\linewidth]{introfig/uncond/flowers/2.jpg}
 \includegraphics[width=0.094\linewidth]{introfig/uncond/flowers/3.jpg}
 \includegraphics[width=0.094\linewidth]{introfig/uncond/flowers/7.jpg}
 \includegraphics[width=0.094\linewidth]{introfig/uncond/flowers/8.jpg}
  \includegraphics[width=0.094\linewidth]{introfig/uncond/flowers/6.jpg}
 \hspace{2mm}
  \raisebox{0.10in}{\rotatebox{90}{\scriptsize \textit{FOOD-101}
 }}
 \includegraphics[width=0.094\linewidth]{introfig/uncond/food/9.jpg}
 \includegraphics[width=0.093\linewidth]{introfig/uncond/food/2.jpg}
 \includegraphics[width=0.093\linewidth]{introfig/uncond/food/3.jpg}
 \includegraphics[width=0.093\linewidth]{introfig/uncond/food/4.jpg}
 \includegraphics[width=0.093\linewidth]{introfig/uncond/food/5.jpg}
\tabularnewline
\hspace{20pt}\captionof{figure}{ \textbf{Qualitative results for unconditional generation by dataset addition above DiT}}
\end{tabular}}
\end{figure*}

==> tookits.tex <==

\usepackage{multirow}
\usepackage{booktabs}
\usepackage{subcaption}
\usepackage{amsmath,amsfonts,bm,amsthm,amssymb}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{graphics,graphicx,caption,float,color}
\usepackage{wrapfig}
\usepackage{bbm}
\usepackage{appendix}

% custom
\usepackage{listings}
\usepackage{xspace}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}} 
\usepackage{hhline}
\usepackage{multicol}
\usepackage{booktabs} 
\usepackage{makecell} % Xhline


% name of our model
\newcommand{\ffn}{TODO Our Method Name}
\newcommand{\ourabbr}{AdaptFormer\xspace}

\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

\definecolor{MyDarkBlue}{rgb}{0,0.08,1}
\definecolor{MyDarkGreen}{rgb}{0.02,0.6,0.02}
\definecolor{MyDarkRed}{rgb}{0.8,0.02,0.02}
\definecolor{MyDarkOrange}{rgb}{0.40,0.2,0.02}
\definecolor{MyPurple}{RGB}{111,0,255}
\definecolor{MyRed}{rgb}{1.0,0.0,0.0}
\definecolor{MyGold}{rgb}{0.75,0.6,0.12}
\definecolor{MyDarkgray}{rgb}{0.66, 0.66, 0.66}

\definecolor{Image}{RGB}{93,59,155}
\definecolor{Video}{RGB}{105,145,60}

\definecolor{ice}{RGB}{84,146,214}
\definecolor{fire}{RGB}{217,129,63}
\definecolor{baselinecolor}{gray}{.9}
\definecolor{poscolor}{RGB}{212,17,89}
\definecolor{negcolor}{RGB}{26,133,255}
\definecolor{bestcolor}{RGB}{238, 255, 238}
% copy-paste from Kaiming's MAE, used for ablation tables
\newcolumntype{x}[1]{>{\centering\arraybackslash}p{#1pt}}
\newcolumntype{y}[1]{>{\raggedright\arraybackslash}p{#1pt}}
\newcolumntype{z}[1]{>{\raggedleft\arraybackslash}p{#1pt}}
% \newcommand{\tablestyle}[2]{\setlength{\tabcolsep}{#1}\renewcommand{\arraystretch}{#2}\centering\footnotesize} % original style from MAE
% \newcommand{\tablestyle}[2]{\setlength{\tabcolsep}{#1}\renewcommand{\arraystretch}{#2}\centering}%\footnotesize


\newcommand{\baseline}[1]{\cellcolor{baselinecolor}{#1}}
\newcommand{\bestcell}[1]{\cellcolor{bestcolor}{#1}}
\newcommand{\aaa}[1]{\textcolor{poscolor}{\small (#1)}}
\newcommand{\bbb}[1]{\textcolor{negcolor}{\small (#1)}}

\newcommand{\rebuttal}[1]{#1}
% \newcommand{\rebuttal}[1]{\textcolor{blue}{#1}}

\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\etal}{\emph{et.al.,}}


